Wide-band view of High Frequency QPOs of GRS 1915+105 in 'softer' variability classes observed with AstroSat

We present a comprehensive temporal and spectral analysis of the 'softer' variability classes ($i.e.$, $\theta$, $\beta$, $\delta$, $\rho$, $\kappa$, $\omega$ and $\gamma$) of the source GRS 1915+105 observed by AstroSat during $2016-2021$ campaign. Wide-band ($3-60$ keV) timing studies reveal the detection of High Frequency Quasi-periodic Oscillations (HFQPOs) with frequency of $68.14-72.32$ Hz, significance of $2.75-11 \sigma$, and rms amplitude of $1.48-2.66\%$ in $\delta$, $\kappa$, $\omega$ and $\gamma$ variability classes. Energy dependent power spectra impart that HFQPOs are detected only in $6-25$ keV energy band and rms amplitude is found to increase ($1-8\%$) with energy. The dynamical power spectra of $\kappa$ and $\omega$ classes demonstrate that HFQPOs seem to be correlated with high count rates. We observe that wide-band ($0.7-50$ keV) energy spectra can be described by the thermal Comptonization component (nthComp) with photon index ($\Gamma_{\rm nth}$) of $1.83-2.89$ along with an additional steep ($\Gamma_{\rm PL}\sim3$) powerlaw component. The electron temperature ($kT_e$) of $1.82 -3.66$ keV and optical depth ($\tau$) of $2-14$ indicate the presence of a cool and optically thick corona. In addition, nthComp components ($1.97 \lesssim \Gamma_{\rm nth} \lesssim 2.44$, $1.06 \times 10^{-8} \lesssim F_{\rm nth} ~({\rm erg} {\rm ~cm}^{-2} {\rm ~s}^{-1}) \lesssim 4.46\times 10^{-8}$) are found to dominate in presence of HFQPOs. Overall, these findings infer that HFQPOs are possibly resulted due to the modulation of the 'Comptonizing corona'. Further, we find that the bolometric luminosity ($0.3-100$ keV) of the source lies within the sub-Eddington ($3-34\%$ $L_{\rm Edd}$) regime. Finally, we discuss and compare the obtained results in the context of existing models on HFQPOs.

==> cover.tex <==
Dear Editor,

I submit the revised version of the manuscript titled 'Wide-band view of High Frequency QPOs of GRS 1915$+$105 in `softer' variability classes observed with AstroSat', ref. MN-21-3623-MJ.R1 . I upload a tar file (allms_03.tar.xz).

The 'allms_03.tar.gz' file contains the followings:

(1) ms_03.pdf, pdf file of manuscripts
(2) ms_03.tex, text file of manuscripts 
(3) fig1.png, figure 1. 
(4) fig2.pdf, figure 2. 
(5) fig3.pdf, figure 3. 
(6) fig4.pdf, figure 4.
(7) fig5.pdf, figure 5.
(8) fig6a.pdf, figure 6a.
(9) fig6b.pdf, figure 6b.
(10) fig7a.pdf, figure 7a.
(11) fig7b.pdf, figure 7b.
(12) fig8.pdf, figure 8.
(13) fig9.pdf, figure 9
(14) Fig_A1.pdf, Appendix figure
(15) cover.tex, a cover letter. 
(16) ms_03.bbl, text file of manuscripts 

With best regards,

Santabrata Das

